Optimal Cost-Preference Trade-off Planning with Multiple Temporal Tasks

Autonomous robots are increasingly utilized in realistic scenarios with multiple complex tasks. In these scenarios, there may be a preferred way of completing all of the given tasks, but it is often in conflict with optimal execution. Recent work studies preference-based planning, however, they have yet to extend the notion of preference to the behavior of the robot with respect to each task. In this work, we introduce a novel notion of preference that provides a generalized framework to express preferences over individual tasks as well as their relations. Then, we perform an optimal trade-off (Pareto) analysis between behaviors that adhere to the user's preference and the ones that are resource optimal. We introduce an efficient planning framework that generates Pareto-optimal plans given user's preference by extending A* search. Further, we show a method of computing the entire Pareto front (the set of all optimal trade-offs) via an adaptation of a multi-objective A* algorithm. We also present a problem-agnostic search heuristic to enable scalability. We illustrate the power of the framework on both mobile robots and manipulators. Our benchmarks show the effectiveness of the heuristic with up to 2-orders of magnitude speedup.

==> sections/1_Introduction.tex <==
\section{Introduction}
\label{sec: intro}

% \ml{\\
% P1: Give the big picture: emphasize high-level tasks... multiple tasks... cost of executing... preference over tasks... This paper aims to develop a computational framework for trade-off analysis between preference and cost of tasks. \\
% P2: Example (Coldtech?) \\
% P3: LTL planning for single tasks - both for mobile robots and manipulators... expressing over task was not included \\
% P4: recent work focus on preference-based planners... WHAT ARE THEIR SHORTCOMINGS? \\
% P5: this work: how do we address those shortcomings????? \\
% P6: Contributions and novelty
% }

% \pa{\\
% contributions:
% 1: pf computation \& single plan synthesis \\
% 2: general preference over costs \\
% 3: heuristics \\
% 4: case studies and benchmarks showing ...}

% \kw{Autonomous robot have advanced into more complex environments. Examples include \ml{examples}.  They are required to plan for multiple tasks while minimizing for time, energy consumption and other objectives. Additionally, robot may need to adhere to human preferences of how the tasks are completed.}

Recent advancements in robotics have enabled robots to take on dominant roles in our daily lives. Examples include self-driving cars, home assistive robots, and cooperative manipulators in factories. 
As they become more integrated into society, there is an increasing demand for them to perform not only multiple simultaneously-assigned complex tasks efficiently (e.g., minimizing time and energy) but also complete them in a way that adheres to human preferences (e.g., some should be completed within a time window and others in a particular order). These objectives, however, are often competing;  that is, by optimizing for efficiency, the execution becomes less preferred.  This results in a trade-off between the objectives, and hence, the goal becomes to optimize for this trade-off.  Nevertheless, there are often many optimal trade-offs, known as the \emph{Pareto front}. \kw{To Morteza: As a reader, it is not clear why computing for all pareto points, i.e., pareto front, is important. Why are we not satisfied with just one pareto point} \jk{I agree with Kandai. Need to explain what "many optimal trade-offs means"}. This poses several challenges from the planning perspective:  
(i) notion of \emph{preference} needs to be formalized, (ii) computation for the whole Pareto front is costly, and (iii) planning space is immensely large due to the multiplicity and complexity of tasks. \jk{Some of these are not worded as "challenges".}
This paper aims to address these challenges by developing an efficient computational framework for analyzing and planning for optimal trade-offs between \textit{cost} and \textit{preference} for multiple complex tasks.
\jk{This is something you say before stating the contributions of the paper. Not before an example.}


% Imagine participating in an activity \kw{activity might be too vague/general.} that requires accomplishing multiple tasks efficiently, such as time, energy/resource consumption, etc. Additionally, the activity also incorporates a preference over how efficiently each individual task is accomplished. Unlike a human, an autonomous robot may not be able to decipher how to efficiently work on several tasks simultaneously, as well as how to complete the tasks in the preferred manner. This paper aims to develop a computational framework for analyzing optimal trade-offs between \textit{cost} and \textit{preference}.
% \kw{I feel like each sentence in this paragraph is not well connected.}

Consider a robotic manipulator working in a restaurant as a cook. The robot receives several food orders. Firstly, the robot should cook all dishes in a minimal time. Secondly, the customers expect that the dishes are served according to the sequence in which each customer placed the order. It is likely that preparing and cooking ingredients simultaneously would be very efficient, but may not respect the order in which the customers should receive their dish. Thus, the robot must determine the appropriate optimal trade-offs between minimizing total cooking time and adhering to the preferred order. 

A popular approach to express complex tasks in robotics is use temporal logics, 
namely \textit{linear temporal logic} (LTL) \cite{BaierBook2008} for its expressive power \cite{Lahijanian:AR-CRAS:2018}. Planning with LTL 
specifications has been widely explored for manipulation applications \cite{He:ICRA:2015,He:IROS:2017,Muvvala:2022:ICRA}, and mobile 
robotic applications \cite{Kress:TRO:2009,Lahijanian:AR-CRAS:2018,Lahijanian:ICRA:2009}. 
Traditionally, a major limitation of those methods is scalability\jk{What does scalability mean here?}.  In addition,
because these applications aim to provide formal guarantees, they fail to reason about preferences or complex soft-constraints \jk{a soft-constraint has not yet been defined. Is this common knowledge?} when planning with multiple tasks. 

Recent work has introduced the notion of 
\ml{several notions?}
\textit{preference} in planning applications
\ml{cite}
. A \textit{preference} can generally be described through qualitative or quantitative measures \cite{jorge2008planning}. \jk{Need an example here of both qualitative and quantitative preferences} Qualitative preferences can be expressed through structures such as a Hierarchical Task Networks \cite{sohrabi2008planning,sohrabi2009htn,sohrabi2010preference,georgievski2014overview} where the user is responsible for qualitatively comparing specification formulae through a binary relation. If the binary relation is \textit{incomplete}, i.e. there exist at least two outcomes that cannot be compared, however, these methods may struggle to reason about temporal objectives. \jk{Previous sentence needs work.} Work \cite{kulkarni2022opportunistic} tackles planning with incomplete preferences over temporal goals, but the quality of the best outcome may be highly dependent on how extensive the user's given binary relation is. Since it may be cumbersome to require the user to provide an extensive binary relation between many outcomes, a natural alternative is to quantify the user's preference. 

Work \cite{bienvenu2006planning} introduces a language to compare qualitative preferences over temporal objectives where the user qualitatively annotates the level of preference for each formula. Similarly, the quantitative preference planning problem can be posed as a partial satisfaction \cite{lahijanian2015time, rahmani2019optimal} or minimum violation/maximum realizability \cite{vasile2017minimum, kamale2021automata, benton2012temporal, mehdipour2020specifying} planning problem. These approaches generally require the user to define costs for certain temporal outcomes based on the tasks alone. Many approaches look to Planning Domain Definition Language (PDDL) \textbf{CITE ORIGINAL PDDL}  to specify quantitative preferences \cite{baier2009heuristic, gerevini2009deterministic, seimetz2021learning}. While these methods provide a framework for reasoning over temporal preferences, they are limited to reasoning about only Boolean temporal behavior, and are unable to reason about the efficiency and performance of the robotic system.

Our approach to synthesizing Pareto optimal plans can be reduced to a bi-objective graph search problem. Recent work builds on a foundational multi-objective $A^*$ search algorithm $NAMOA^*$ which determines the Pareto-optimal solution set of \textit{non-dominated} paths. For these problems, each objective is captured by an element in a cost vector that ``weights'' each edge. Unlike scalar edge weights, two cost vectors have no intrinsic binary relation, thus algorithms based on $NAMOA^*$ rely on an incomplete comparison known as \textit{dominance}. 

\ml{need a paragraph on multi-objective planning! Use the following paragraph as a guide... need to rephrase it... As look at the citations and see how they're different from yours:  \\ \\
Multi-objective path planning (MOPP) problems in graphs: \\
Given a graph where each edge is associated with a non- negative cost vector (where each component of the vector corresponds to an objective), MOPP aims to find a set of Pareto-optimal (also called non-dominated) paths connecting the given start and destination vertex in the graph. MOPP has been studied for decades [1,2] and remains an active research area [3-5]. Conventionally, this problem has been regarded as computationally expensive especially when there are many Pareto-optimal paths. 
The recent advances in Multi-Objective A* (MOA*)- like algorithms [3,4] expedite the search and make it possible to employ MOA* as a sub- routine to solve more complicated planning problems.\\ \\
- [1] Loui, R. P. 1983. Optimal paths in graphs with stochastic or multidimensional weights. Communications of the ACM, 26(9): 670–676. \\
- [2] Mandow, L.; and De La Cruz, J. L. P. 2008. Multiobjective A* search with consistent heuristics. Journal of the ACM (JACM), 57(5): 1–25.\\
- [3] Ren, Z.; Zhan, R.; Rathinam, S.; Likhachev, M.; and Choset, H. 2022. Enhanced Multi-Objective A* Using Balanced Bi- nary Search Trees. In Proceedings of the International Sym- posium on Combinatorial Search, volume 15, 162–170.\\
- [4] Ulloa, C. H.; Yeoh, W.; Baier, J. A.; Zhang, H.; Suazo, L.; and Koenig, S. 2020. A simple and fast bi-objective search algorithm. In Proceedings of the International Conference on Automated Planning and Scheduling, volume 30, 143– 151.\\
- [5] Zhang, H.; Salzman, O.; Kumar, T. K. S.; Felner, A.; Hernandez Ulloa, C.; and Koenig, S. 2022. A*pex: Efficient Approximate Multi-Objective Search on Graphs. Proceed- ings of the International Conference on Automated Planning and Scheduling, 32(1): 394–403.
}

This work aims to provide a new perspective on preference-based planning that allows the user to express a preference with respect to the (cost) behavior of an actual robotic system. In our framework, it is assumed that all individual tasks must be completed, and the user can express their preference over the cumulative cost of completing each task in relation to the other tasks. Under this novel preference formulation, an optimal trade-off analysis can be performed to illustrate the robot's behavior for varying levels of preference adhesion.
\ml{also need to give an overview of the computational framework here!}

\jk{It would be helpful to the reader to map this papers "contributions" back to the "challenges" states above. Consider re-writing.}
The contributions of this paper are as follows. Firstly, we formalize a novel \kw{generalized} notion of preference over the cost of satisfying each individual task. Second, given the user's preference, we introduce an algorithm for synthesizing a plan given a preference constraint, as well as an algorithm for computing all optimal trade-off plans. Third, since both algorithms suffer from poor scalability with large problems, we define a problem-agnostic heuristic to speed up the computation time considerably. Lastly, we demonstrate the power of our preference notion using case studies, as well as the effectiveness of the heuristic using benchmarks.




==> sections/2_Preliminaries.tex <==
\subsection{}
\label{sec: preliminaries}

